Signer-Optimal Multiple-Time Post-Quantum Hash-Based Signature for Heterogeneous IoT Systems

Heterogeneous Internet of Things (IoTs) harboring resource-limited devices like wearable sensors are essential for next-generation networks. Ensuring the authentication and integrity of security-sensitive telemetry in these applications is vital. Digital signatures provide scalable authentication with non-repudiation and public verifiability, making them essential tools for IoTs. However, emerging quantum computers necessitate post-quantum (PQ) secure solutions, yet existing NIST-PQC standards are costlier than their conventional counterparts and unsuitable for resource-limited IoTs. There is a significant need for lightweight PQ-secure digital signatures that respect the resource constraints of low-end IoTs. We propose a new multiple-time hash-based signature called Maximum Utilization Multiple HORS (MUM-HORS) that offers PQ security, short signatures, fast signing, and high key utilization for an extended lifespan. MUM-HORS addresses the inefficiency and key loss issues of HORS in offline/online settings by introducing compact key management data structures and optimized resistance to weak-message attacks. We tested MUM-HORS on two embedded platforms (ARM Cortex A-72 and 8-bit AVR ATmega2560) and commodity hardware. Our experiments confirm up to 40x better utilization with the same signing capacity (2^20 messages, 128-bit security) compared to multiple-time HORS while achieving 2x and 156-2463x faster signing than conventional-secure and NIST PQ-secure schemes, respectively, on an ARM Cortex. These features make MUM-HORS ideal multiple-time PQ-secure signature for heterogeneous IoTs.

==> Backup.tex <==
\begin{algorithm}[H]
    \footnotesize
    \caption{Maximum Utilization Multiple HORS (MUM-HORS)}\label{alg:mumhors}
    \hspace{5pt}
     
    %%%%%%%% Keygen %%%%%%%%
    \begin{algorithmic}[1]
        \vspace{-5pt}
        \Statex $ \underline{ (\sk, \pk, \bitmap, I_{\mumhors}) \as \mumhorskg(1^{\kappa}) } $:
        \vspace{-1pt}
        \State Set $I_{\mumhors} \as (I_{\hors}, r, rt)$, $msk \Ra \{0,1\}^\kappa$, and $\{pad_{i}\}_{i=1}^3$

        \State Build bitmap $\bitmap = \{row_i\}_{i=1}^{rt}$ and set $row_i.num = i$, $row_i.activebits = t$, $row_i.next = row_{i+1}$, all $row_i.bits[.]$ to 1, and $row_{rt}.next = \bot$. Set $\bitmap.head = row_1$, $\bitmap.tail = row_{rt}$, $\bitmap.window = t$, $\bitmap.nextrow = rt+1$, $\bitmap.activerows = rt$, and $\bitmap.activebits = rt\times t$. 

        \State Create public keys $\pk \!\!\as\!\! \{pk_{i}\}_{i=1}^r$ and set $pk_i.num = i$, $pk_i.activepk = t$, $pk_i.next = pk_{i+1}$, $\{pk_i.keys[j] \!\!\!\as\!\!\! f(PRF(msk || i || j))\}_{\substack{1 \leq i \leq r , 1 \leq j \leq t}}$, and $pk_{r}.next = \bot$. Set $\pk.head = pk_1$, $\pk.tail = pk_{rt}$, $\pk.window = t$, $\pk.nextrow = rt+1$, $\pk.activerows = rt$, and $\pk.activepks = rt\times t$.

        \State Send the private key $\sk \as msk$ and $\bitmap$ to the signer, store the public keys $\pk$ on the verifier, and output the $I_{\mumhors}$
    \end{algorithmic}
    \algrule


    %%%%%%%%% Sign %%%%%%%%
    \begin{algorithmic}[1]
        \vspace{-5pt}
        \Statex $\underline{\sigma\as \mumhorssig(\sk, m)}$: Setting $Ctr = 0$ and $hash \as H(m)$
        \vspace{3pt}

        \State $hash' \as H ( hash || Ctr )$ and $hash'' \as Trunc(hash', k\log t)$
        \State Split $hash''$ into $k$ substrings  $ \{ hash''_j \}_{j = 1}^{k} $ s.t. $ |hash''_j| = \log t $		
        \State Interpret each $hash''_j$ as an integer $i_j$,  $ \forall j  \in [1, k]$
        \State \textbf{if} {exist $p,q \in [1, k]$ s.t. $i_p = i_q$ and $p\neq q$} \textbf{then} $Ctr = Ctr+1$ and \textbf{goto} step 1 
        \State Compute $\{(r_j, c_j)\} \as \bitmapgetrowcol(\bitmap, i_j)$, $\forall j \in [1, k]$    
        \State \Return  $\sigma \as (\{ PRF(sk || r_j || c_j) \}_{j = 1}^k, Ctr)$
        \algsep{\textit{Signer is idle}}
        \State $\bitmapunsetindices(\bitmap, i_j)$, $\forall j \in [1, k]$
        \If {\bitmapextendmatrix(\bitmap) == $\smallfalse$} No more private keys to sign and \textbf{exit} \EndIf
    \end{algorithmic}
    \algrule

    %%%%%%%% Verify %%%%%%%%
    \begin{algorithmic}[1]
        \vspace{-5pt}
        \Statex $ \underline{ b \as \mumhorsver( \pk, m, \sigma)}$: Setting $hash \as H(m)$
        \vspace{3pt}
        \State $hash' \as H(hash || Ctr)$ and $hash'' \as Trunc(hash', k\log t)$
        \State Split $hash''$ into $k$ substrings  $ \{ hash''_j \}_{j = 1}^{k} $ s.t. $ |hash''_j| = \log t $	
        \State Interpret each $hash''_j$ as an integer $i_j$, $\forall j \in [1, k]$
        \State \textbf{if} {exist $p,q \in [1, k]$ s.t. $i_p = i_q$ and $p\neq q$} \textbf{then} Find the correct $Ctr$ as in $\mumhorssig(.)$ and the indices $i_j$ and \textbf{return} $b=0$. 
        \State Retrieve non-$\bot$ public key $pk_j$ for every index $i_j$ similar to $\bitmapgetrowcol(.)$ and if $(pk_j \neq f(\sigma_j))$ \textbf{return} $b=0$, $ \forall j  \in [1, k]$. Otherwise, \textbf{return} $b=1$
        \algsep{\textit{Verifier is idle}}
        \State Invalidate all the $pk_j$ corresponding to the derived $i_j$ similar to $\bitmapunsetindices(.)$ by setting them to $\bot$ and \textbf{return} $b$
        \State Extend the view of the public keys similar to $\bitmapextendmatrix(.)$
    \end{algorithmic}
\end{algorithm}



\begin{algorithm}[H]
    \footnotesize
    \caption{Bitmap Manipulation Algorithms using Circular Queue}\label{alg:mumhorsarray}
    \hspace{5pt} 
    \scriptsize
    %%%%%%%%%% BITMAP EXTEND %%%%%%%%%%
    \begin{algorithmic}[1]
        \vspace{-5pt}
	\Statex $b \as \underline{\bitmapextendmatrix (\bitmap)}$:
        % \vspace{-1pt}
        \If{$\bitmap.activebits < \bitmap.window$}
            \If{$\bitmap.nextrow \ge r$} \Return $\smallfalse$ \EndIf
            
            \If {$\bitmapcleanup(\bitmap) == 0$}
                \State Set $index$ to the index of the row with the minimum $.activebits$
                \State $\bitmap.activerows \minusEquals 1$ and $\bitmap.activebits \minusEquals \bitmap[i].activebits$
                \State $\bitmapremoverow(index)$
                \EndIf
            \State $fillcapacity = min(rt - \bitmap.activerows, r - \bitmap.nextrow)$        
            \State Add $fillcapacity$ rows to $\bitmap$ by creating new $row$ and and setting $\bitmap[i].num = \bitmap.nextrow$, $\bitmap[i].activebits = t$, all $\bitmap[i].bits[.]$ to 1, $\bitmap[tail] = row$, $\bitmap.nextrow \plusEquals 1 \mod rt$ and $\bitmap.tail \plusEquals 1 \mod rt$ for each.
        \EndIf
            \State \Return $\smalltrue$ 
    \end{algorithmic}
    \algrule

    %%%%%%%%%% BITMAP CLEANUP %%%%%%%%%%
    \begin{algorithmic}[1]
	\Statex $n \as \underline{\bitmapcleanup(\bitmap)}$: Set $cleaned = 0$
        \If{$\bitmap.tail > \bitmap.head$}
            \For{$i \!\!=\!\! \bitmap.head$ to $\bitmap.tail$} \textbf{if}~{$\bitmap[i].activebits \!==\! 0$} \textbf{then} $\bitmapremoverow(i)$ and $cleaned \plusEquals 1$ \EndFor
        \Else
            \For{$i = \bitmap.head$ to $rt$} \textbf{if}~{$\bitmap[i].activebits == 0$} \textbf{then} $\bitmapremoverow(i)$ and $cleaned \plusEquals 1$ \EndFor
            \For{$i = 0$ to $\bitmap.head$} \textbf{if}~{$\bitmap[i].activebits == 0$} \textbf{then} $\bitmapremoverow(i)$ and $cleaned \plusEquals 1$ \EndFor
        \EndIf
        \State \Return $cleaned$
    \end{algorithmic}
    \algrule
    
    %%%%%%%%%% BITMAP Get Row and Col %%%%%%%%%%
    \begin{algorithmic}[1]
        \Statex $(row, col) \as \underline{\bitmapgetrowcol(\bitmap, index)}$: %Set global $i=0$
        
        \If{$\bitmap.tail > \bitmap.head$}
            \For{$i = \bitmap.head$ to $\bitmap.tail$} \textbf{if}~{$index \ge \bitmap[i].activebits$} \textbf{then} $index \minusEquals \bitmap[i].activebits$ \EndFor
        \Else
            \For{$i = \bitmap.head$ to $rt$} \textbf{if}~{$index \ge \bitmap[i].activebits$} \textbf{then} $index \minusEquals \bitmap[i].activebits$ \textbf{else} \textbf{goto} 6\EndFor
            \For{$i = 0$ to $\bitmap.head$} \textbf{if}~{$index \ge \bitmap[i].activebits$} \textbf{then} $index \minusEquals \bitmap[i].activebits$ \textbf{else} \textbf{goto} 6 \EndFor
        \EndIf
        \State Set $colidx$ as the index of $(index+1)^{th}$ set bit in $\bitmap[i].bits[.]$ and \textbf{return} $(\bitmap[i].num, colidx)$
    \end{algorithmic}
    \algrule
    
    \begin{algorithmic}[1]
        \Statex $\underline{\bitmapunsetindices(\bitmap, \indices)}$: Set $delta = 0$
        \State Sort $\indices$ and \textbf{if} {$\indices[i] \neq \indices[i-1]$} \textbf{then} $\indices[i] \minusEquals delta$ and $delta \plusEquals 1$ 
        \For{$index$ \textbf{in} $\indices$}
            % \State Set global $i=0$
            \If{$\bitmap.tail \ge \bitmap.head$}
                \For{$i = \bitmap.head$ to $\bitmap.tail$} \textbf{if}~{$index \ge \bitmap[i].activebits$} \textbf{then} $index \minusEquals \bitmap[i].activebits$ \EndFor
            \Else
                \For{$i = \bitmap.head$ to $rt$} \textbf{if}~{$index \ge \bitmap[i].activebits$} \textbf{then} $index \minusEquals \bitmap[i].activebits$ \textbf{else} \textbf{goto} 8\EndFor
                \For{$i = 0$ to $\bitmap.head$} \textbf{if}~{$index \ge \bitmap[i].activebits$} \textbf{then} $index \minusEquals \bitmap[i].activebits$ \textbf{else} \textbf{goto} 8 \EndFor
            \EndIf
            \State Unset the $(index+1)^{th}$ bit in $\bitmap[i].bits[.]$ to 0
            \State Update $\bitmap.activebits \minusEquals 1$ {and} $\bitmap[i].activebits \minusEquals 1$
        \EndFor             
    \end{algorithmic}
    \algrule
    \begin{algorithmic}[1]
    \Statex $\underline{\bitmapremoverow(index)}$: 
        \If{$\bitmap.tail > \bitmap.head$}

            \If{$index < \frac{\bitmap.tail - \bitmap.head}{2}$} 
                Shift right all rows from $\bitmap.head$ to $\bitmap.head+index$ and set $\bitmap.head = index$
            \Else
                 \hspace{0.1mm} Shift left all rows from $\bitmap.tail$ to $\bitmap.head+index$ and set $\bitmap.tail = index$ 
            \EndIf
        \Else
            \If{$\bitmap.head + index < rt$} 
                Shift right all rows from $\bitmap.head$ to $\bitmap.head+index$ and set $\bitmap.head = index$
            \Else
                \hspace{0.1mm} Shift left all rows from $\bitmap.tail$ to $\bitmap.tail-rt+index$ and set $\bitmap.tail = index$ 
            \EndIf      
        \EndIf
        \State \Return $cleaned$
    \end{algorithmic}
    
\end{algorithm}






% \begin{algorithm}[H]
%     \footnotesize
%     \caption{Bitmap Manipulation Algorithms}\label{alg:bitmap}
%     \hspace{5pt}
%     %%%%%%%%%% BITMAP EXTEND %%%%%%%%%%
%     \begin{algorithmic}[1]
%         \vspace{-5pt}
% 	\Statex $b \as \underline{\bitmapextendmatrix (\bitmap)}$:
%         \If{$\bitmap.activebits < \bitmap.window$}
%             \If{$\bitmap.nextrow > r$} \Return $\smallfalse$ \EndIf
%             \If {$\bitmapcleanup(\bitmap) == 0$}  %\Comment{No row was removed, so choose the best }
%                 \State Set $row$ to the row with the minimum $activebits$ parameter
%                 \State Update $\bitmap.activerows \minusEquals 1$ and $\bitmap.activebits \minusEquals row.activebits$
%                 \State Remove $row$ from $\bitmap$
%             \EndIf
%             \State $fillcapacity = min(rt - \bitmap.activerows, r - \bitmap.nextrow)$
%             \State Add $fillcapacity$ rows to $\bitmap$ by creating new $row$ and setting $row.num = \bitmap.nextrow$, $row.activebits = t$, all $row.bits[.]$ to 1, $row.next = \bot$, $\bitmap.tail.next = row$ and $\bitmap.nextrow \plusEquals 1$ for each.
%         \EndIf
%             \State \Return $\smalltrue$ 

%     \end{algorithmic}
%     \algrule

%     %%%%%%%%%% BITMAP CLEANUP %%%%%%%%%%
%     \begin{algorithmic}[1]
% 	\Statex $n \as \underline{\bitmapcleanup(\bitmap)}$: Set $cleaned = 0$ and $row = \bitmap.head$
%         \While{$row$ is not $\bot$} 
%             \If{$row.activebits$ == 0} \State Remove $row$ from $\bitmap$ and set $cleaned \mathrel{+}= 1$ and $row = row.next$ \EndIf
%         \EndWhile
%         \State \Return $cleaned$
%     \end{algorithmic}
%     \algrule
%     %%%%%%%%%% BITMAP Get Row and Col %%%%%%%%%%
%     \begin{algorithmic}[1]
%         \Statex $(row, col) \as \underline{\bitmapgetrowcol(\bitmap, index)}$: Set $row = \bitmap.head$
%         \While{$row$ is not $\bot$}
%             \If{$index < row.activebits$} \textbf{break} \EndIf
%             \State Update $index \minusEquals row.activebits$ and $row = row.next$
%         \EndWhile
%         \State Set $colidx$ as the index of $(index+1)^{th}$ set bit in $row.bits[.]$ and \textbf{return} $(row.num, colidx)$
%     \end{algorithmic}
%     \algrule
    
%     \begin{algorithmic}[1]
%         \Statex $\underline{\bitmapunsetindices(\bitmap, \indices)}$: Set $delta = 0$
%         \State Sort $\indices$ and \textbf{if} {$\indices[i] \neq \indices[i-1]$} \textbf{then} $\indices[i] \minusEquals delta$ and $delta \plusEquals 1$ 
        
%         \For{$index$ \textbf{in} $\indices$}
%             \State $row = \bitmap.head$
%             \While{$row$ is not $\bot$}
%                 \If{$index < row.activebits$} \textbf{break} \EndIf
%                 \State $index  \minusEquals row.activebits$ {and} $row = row.next$
%             \EndWhile

%             \State Unset the $(index+1)^{th}$ bit in $row.bits[.]$ to 0
%             \State Update $\bitmap.activebits \minusEquals 1$ {and} $row.activebits \minusEquals 1$
%         \EndFor  
%     \end{algorithmic}
% \end{algorithm}


==> notes.tex <==






Commidity Array

================ MUM-HORS Report ================
Accepted signatures: 2/1048576 (1048574 rejected)
-- Total Sign time (w rejection sampling w.o. bitmap): 12.890784999934 s
-- Total Verify time (w rejection checking): 15.401108999754 s 
-- Each sign time (w rejection sampling w.o. bitmap): 12.293610572752 micros
-- Each verify time (w rejection checking): 14.687642097239 micros

================ Bitmap Report ================
#ROW_ALLOC(.): 7328
	#ROW_CLEANUP(.): 7327
		--- Empty rows removed: 25590
	#ROW_DIRECT_REMOVE(.): 2
#INDEX_GET_ROW_COL(.)/Index: 26214400
#INDEX_UNSET(.)/Batch: 1048576
--- Discarded rows: 2/25601
--- Discarded bits: 2/26215424

------- Timings -------
--- TT Cleanup: 746.000000000011 micros
--- TT Direct Remove Row: 844.000000000012 micros
--- TT Get Row Col: 6409711.000539560802 micros
--- TT Unset Bits: 5121177.999918602407 micros

--- AVGT Cleanup: 0.029152012505 micros
--- AVGT Direct Remove Row: 0.032979055955 micros
--- AVGT Get Row Col: 0.244511070272 micros
--- AVGT Unset Bits: 4.883935928267 micros



Commidity List

[INF] Generating the public keys ...
KEYGEN: 10.432417000000
[INF] Running the test cases ...
[1048575/1048576][INF] 

[Signer] No more rows are left to sign

================ MUM-HORS Report ================
Accepted signatures: 2/1048576 (1048574 rejected)
-- Total Sign time (w rejection sampling w.o. bitmap): 12.504947999967 s
-- Total Verify time (w rejection checking): 14.551166999775 s 
-- Each sign time (w rejection sampling w.o. bitmap): 11.925647735564 micros
-- Each verify time (w rejection checking): 13.877074241424 micros

================ Bitmap Report ================
#ROW_ALLOC(.): 7328
	#ROW_CLEANUP(.): 7327
		--- Empty rows removed: 25590
	#ROW_DIRECT_REMOVE(.): 2
#INDEX_GET_ROW_COL(.)/Index: 26214400
#INDEX_UNSET(.)/Batch: 1048576
--- Discarded rows: 2/25601
--- Discarded bits: 2/26215424

------- Timings -------
--- TT Cleanup: 1607.999999999969 micros
--- TT Direct Remove Row: 0.000000000000 micros
--- TT Get Row Col: 6115581.000498134643 micros
--- TT Unset Bits: 5073051.999919898808 micros

--- AVGT Cleanup: 0.062837045721 micros
--- AVGT Direct Remove Row: 0.000000000000 micros
--- AVGT Get Row Col: 0.233290901203 micros
--- AVGT Unset Bits: 4.838039398117 micros








ARM Array
'[INF] Generating the public keys ...
KEYGEN: 74.792526000000
[INF] Running the test cases ...
[1048575/1048576][INF] 

[Signer] No more rows are left to sign

================ MUM-HORS Report ================
Accepted signatures: 2/1048576 (1048574 rejected)
-- Total Sign time (w rejection sampling w.o. bitmap): 96.116139000081 s
-- Total Verify time (w rejection checking): 77.578369000648 s 
-- Each sign time (w rejection sampling w.o. bitmap): 91.663493156510 micros
-- Each verify time (w rejection checking): 73.984498024605 micros

================ Bitmap Report ================
#ROW_ALLOC(.): 7328
        #ROW_CLEANUP(.): 7327
                --- Empty rows removed: 25590
        #ROW_DIRECT_REMOVE(.): 2
#INDEX_GET_ROW_COL(.)/Index: 26214400
#INDEX_UNSET(.)/Batch: 1048576
--- Discarded rows: 2/25601
--- Discarded bits: 2/26215424

------- Timings -------
--- TT Cleanup: 11299.999999999744 micros
--- TT Direct Remove Row: 21225.999999999607 micros
--- TT Get Row Col: 38864251.995653264225 micros
--- TT Unset Bits: 22344410.000055234879 micros

--- AVGT Cleanup: 0.441578741696 micros
--- AVGT Direct Remove Row: 0.829399812441 micros
--- AVGT Get Row Col: 1.482553558184 micros
--- AVGT Unset Bits: 21.309289932304 micros





ARM List


[INF] Generating the public keys ...
KEYGEN: 78.388285000000
[INF] Running the test cases ...
[1048575/1048576][INF] 

[Signer] No more rows are left to sign

================ MUM-HORS Report ================
Accepted signatures: 2/1048576 (1048574 rejected)
-- Total Sign time (w rejection sampling w.o. bitmap): 96.574983000052 s
-- Total Verify time (w rejection checking): 77.515219000618 s 
-- Each sign time (w rejection sampling w.o. bitmap): 92.101080894519 micros
-- Each verify time (w rejection checking): 73.924273491495 micros

================ Bitmap Report ================
#ROW_ALLOC(.): 7328
        #ROW_CLEANUP(.): 7327
                --- Empty rows removed: 25590
        #ROW_DIRECT_REMOVE(.): 2
#INDEX_GET_ROW_COL(.)/Index: 26214400
#INDEX_UNSET(.)/Batch: 1048576
--- Discarded rows: 2/25601
--- Discarded bits: 2/26215424

------- Timings -------
--- TT Cleanup: 10863.999999999984 micros
--- TT Direct Remove Row: 2.000000000000 micros
--- TT Get Row Col: 38832120.995531223714 micros
--- TT Unset Bits: 24607926.000014640391 micros

--- AVGT Cleanup: 0.424540836264 micros
--- AVGT Direct Remove Row: 0.000078149422 micros
--- AVGT Get Row Col: 1.481327857801 micros
--- AVGT Unset Bits: 23.467947006240 micros



